Balancing Shared and Task-Specific Representations: A Hybrid Approach to Depth-Aware Video Panoptic Segmentation

In this work, we present Multiformer, a novel approach to depth-aware video panoptic segmentation (DVPS) based on the mask transformer paradigm. Our method learns object representations that are shared across segmentation, monocular depth estimation, and object tracking subtasks. In contrast to recent unified approaches that progressively refine a common object representation, we propose a hybrid method using task-specific branches within each decoder block, ultimately fusing them into a shared representation at the block interfaces. Extensive experiments on the Cityscapes-DVPS and SemKITTI-DVPS datasets demonstrate that Multiformer achieves state-of-the-art performance across all DVPS metrics, outperforming previous methods by substantial margins. With a ResNet-50 backbone, Multiformer surpasses the previous best result by 3.0 DVPQ points while also improving depth estimation accuracy. Using a Swin-B backbone, Multiformer further improves performance by 4.0 DVPQ points. Multiformer also provides valuable insights into the design of multi-task decoder architectures.

==> tikz/nnfeature.tex <==
%auto-ignore
\makeatother
\tikzset{
nnfeature/.style={
    rectangle, 
    minimum width=14mm,
    minimum height=8mm,
    fill=nnfeatureFillColor,
    draw=nnfeatureFillColor!60!black, thin, 
    font=\small\linespread{0.8}\selectfont\vphantom{Ag},
},
% Set of nnfeatures
nnfeatureset/.style={
    path picture={
        \foreach \i in {\nnfeatureset@layers,...,1}{
            \node [
                 draw=\nnfeatureset@draw, thick,
                 fill=\nnfeatureset@fill\i!70!white,%\nnfeatureset@fill,
                 inner sep=0, 
                 minimum width=\nnfeatureset@width, 
                 minimum height=\nnfeatureset@height,
                 yshift=(\i-\nnfeatureset@layers+1) * \nnfeatureset@ysep,
                 xshift=(\i-\nnfeatureset@layers+1) * \nnfeatureset@xsep,
            ] 
            (-layer\i) at (0, 0) {\nnfeatureset@label};
        }
    },
    minimum width=\nnfeatureset@width + \nnfeatureset@layers*\nnfeatureset@xsep + \pgflinewidth,
    minimum height=\nnfeatureset@height +\nnfeatureset@layers*\nnfeatureset@ysep + \pgflinewidth,
    anchor=center,
},
nnfeatureset height/.store in=\nnfeatureset@height,
nnfeatureset width/.store in=\nnfeatureset@width,
nnfeatureset layers/.store in=\nnfeatureset@layers,
nnfeatureset label/.store in=\nnfeatureset@label,
nnfeatureset xsep/.store in =\nnfeatureset@xsep,
nnfeatureset ysep/.store in =\nnfeatureset@ysep,
nnfeatureset fill/.store in =\nnfeatureset@fill,
nnfeatureset draw/.store in =\nnfeatureset@draw,
nnfeatureset width=1cm,
nnfeatureset height=1cm,
nnfeatureset layers=4,
nnfeatureset xsep=1mm,
nnfeatureset ysep=1mm,
nnfeatureset fill=QueryColor,
nnfeatureset label={},
nnfeatureset draw=DrawColor,
% Multi-level nnfeatures
nnmultifeature/.style={
    path picture={
        \foreach \i in {1,...,\nnmultifeature@layers}{
            \node [
                 draw=\nnmultifeature@draw,
                 fill=\nnmultifeature@fill,
                 inner sep=0, 
                 minimum width=\nnmultifeature@width - ((\i-1) * 0.75 * \nnmultifeature@width/\nnmultifeature@layers)), 
                 minimum height=\nnmultifeature@height,
                 yshift=(\i-1) * (\nnmultifeature@sep + \nnmultifeature@height) - (\nnmultifeature@sep * (\nnmultifeature@layers-1) + \nnmultifeature@height * (\nnmultifeature@layers - 1)) * 0.5,
            ] 
            (-layer\i) at (0, 0) {};
        }
    },
    minimum width=\nnmultifeature@width + \pgflinewidth,
    minimum height=(\nnmultifeature@height * \nnmultifeature@layers) + (\nnmultifeature@sep * (\nnmultifeature@layers-1)) + \pgflinewidth,
},
nnmultifeature height/.store in=\nnmultifeature@height,
nnmultifeature width/.store in=\nnmultifeature@width,
nnmultifeature layers/.store in=\nnmultifeature@layers,
nnmultifeature sep/.store in =\nnmultifeature@sep,
nnmultifeature fill/.store in =\nnmultifeature@fill,
nnmultifeature draw/.store in =\nnmultifeature@draw,
nnmultifeature width=10mm,
nnmultifeature height=2mm,
nnmultifeature layers=4,
nnmultifeature sep=0.5mm,
nnmultifeature fill=FeatureFillColor,
nnmultifeature draw=black,
}
\makeatletter

==> tikz/nnquery.tex <==
%auto-ignore

% define some methods for drawing queries in NN diagrams
%
% 2024-09-5 stolle
%
% Query colors
\definecolor{NNQueryColor1}{HTML}{05D6ED}
\definecolor{NNQueryColor2}{HTML}{D94032} 
\definecolor{NNQueryColor3}{HTML}{F2E41D}
\definecolor{NNQueryColor4}{HTML}{CAF21D}
\makeatletter
\tikzset{
  nnquery/.pic={
     code={%
      \begin{scope}[align=center, anchor=center]
          \node[%
                %fill=black!10, draw=black!30, 
                rounded corners=\nnquery@padding,
                draw=black!1!white,
                line width=\nnquery@padding,
                outer sep=0,%\nnquery@padding,
                text centered,
                text width=0,
                anchor=center,
                inner sep=0,
                shape=rectangle split, 
                rectangle split parts=\nnquery@dim, 
                rectangle split horizontal,
                rectangle split part fill={NNQueryColor1,NNQueryColor2,NNQueryColor3,NNQueryColor4},
                rectangle split ignore empty parts=false,
                rectangle split part align=center,%
                rectangle split empty part width=0,%\nnquery@width,
                rectangle split empty part height=\nnquery@height,
                rectangle split empty part depth=0ex,%\nnquery@height,
          ] (-vectors) at (0,0) {};
          \node[draw=black!60!white,thin,rounded corners=\nnquery@padding,fit=(-vectors),inner sep=0] (-box) {};
      \end{scope}
    }
  },
  nnquery dim/.store in=\nnquery@dim,
  nnquery dim=4,
  nnquery height/.store in=\nnquery@height,
  nnquery height=3mm,
  nnquery width/.store in=\nnquery@width,
  nnquery width=1mm,
  nnquery padding/.store in=\nnquery@padding,
  nnquery padding=1.25pt,
}
\makeatother

==> tikz/path.ortho.tex <==
%auto-ignore

%% For the operators r-lr, r-rl, r-ud and r-du we need to check after TikZ found r
\let\tikz@orig@rect\tikz@rect
\def\tikz@rect{\pgfutil@ifnextchar e\tikz@orig@rect\tikzext@tikz@r}
\def\tikzext@tikz@r -{%
  \pgfutil@ifnextchar l\tikzext@tikz@lr@lineto{%
    \pgfutil@ifnextchar r\tikzext@tikz@rl@lineto{%
      \pgfutil@ifnextchar u\tikzext@tikz@ud@lineto{%
        \pgfutil@ifnextchar d\tikzext@tikz@du@lineto\tikz@expand
      }%
    }%
  }%
}
%% For the operator |-| we need to check after TikZ found |-
\let\tikz@orig@vh@lineto@next\tikz@vh@lineto@next
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar|{\expandafter\tikzext@tikz@vhv@lineto\pgfutil@gobble}%
    {\pgfutil@ifnextchar\tikz@activebar{\expandafter\tikzext@tikz@vhv@lineto\pgfutil@gobble}%
      {\tikz@orig@vh@lineto@next}}}
%% For the operator -|- we need to check after TikZ found -|
\let\tikz@orig@hv@lineto\tikz@hv@lineto
\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar-{\expandafter\tikzext@tikz@hvh@lineto\pgfutil@gobble}%
    {\tikz@orig@hv@lineto}}

%% |-|[<opts>] and -|-[<opts>] are allowed
\def\tikzext@tikz@vhv@lineto{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@vhv@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@vhv@lineto@next[]}}
\def\tikzext@tikz@hvh@lineto{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@hvh@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@hvh@lineto@next[]}}

%% r-rl[<opts>], r-lr[<opts>], etc.
\def\tikzext@tikz@rl@lineto rl{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@rl@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@rl@lineto@next[]}}
\def\tikzext@tikz@lr@lineto lr{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@lr@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@lr@lineto@next[]}}
\def\tikzext@tikz@du@lineto du{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@du@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@du@lineto@next[]}}
\def\tikzext@tikz@ud@lineto ud{\pgfutil@ifnextchar[{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@ud@lineto@next}{\tikzext@tikz@collect@hvvh@options\tikzext@tikz@ud@lineto@next[]}}

%% TikZ interjects are done, the rest is independent:


\newdimen\tikzext@tikz@udlr@distance
\newdimen\tikzext@tikz@hvvh@distance
\newif\iftikzext@tikz@hvvh@middle         % checks whether spacing = 0 was selected
\newif\iftikzext@tikz@hvvh@fromcenter
\newif\iftikzext@ortho@preflush
\tikzext@ortho@preflushtrue

%%% HVVH/UDLR
\tikzset{%
  ortho/.code=\pgfqkeys{/tikz/ortho}{#1},
  hvvh/.code=\pgfqkeys{/tikz/ortho}{#1},%
  udlr/.code=\pgfqkeys{/tikz/ortho}{#1},%
  ortho/.search also=/tikz,
  ortho/middle 0 to 1/.style={/tikz/ortho/spacing=0},%
  ortho/from center/.is if=tikzext@tikz@hvvh@fromcenter,%
  ortho/spacing/.code=% spacing = 0 means that the middle part are the pos-itions 0 to 1,
  %                                           the first part is -1 to 0, the last part is to 2
    \pgfmathint{#1}\let\tikzext@tikz@hvvh@timing@parts\pgfmathresult% in case they are calculations to be done
    \ifcase\tikzext@tikz@hvvh@timing@parts\relax
      \tikzext@tikz@hvvh@middletrue
      \def\tikzext@tikz@hvvh@timing@parts{1}%
      \def\tikzext@tikz@hvvh@timing@first{0}%
      \def\tikzext@tikz@hvvh@timing@last{1}%
      \def\tikzext@tikz@hvvh@timing@subtr{0}%
      \def\tikzext@tikz@hvvh@timing@factor{1}%
    \else            % in all other cases n > 0 the kinks are at pos = 1/n and (n - 1)/n
      \tikzext@tikz@hvvh@middlefalse
      \pgfmathreciprocal{#1}\let\tikzext@tikz@hvvh@timing@first\pgfmathresult
      \pgfmathsetmacro\tikzext@tikz@hvvh@timing@last{1-\pgfmathresult}%
      \pgfmathreciprocal{#1-2}%
      \let\tikzext@tikz@hvvh@timing@subtr\pgfmathresult
      \pgfmathsetmacro\tikzext@tikz@hvvh@timing@factor{1+2*\pgfmathresult}%
    \fi,%
  ortho/ratio/.code=\pgfmathsetmacro\tikzext@tikz@hvvh@ratio{#1},%
  % TODO: not possible to do distance in TikZ coordinate system
  ortho/distance/.code=\pgfmathsetlength\tikzext@tikz@hvvh@distance{#1}\let\tikzext@tikz@hvvh@ratio\pgfutil@empty,%
  ortho/udlr distance/.style={%
    /tikz/ortho/ud distance={#1},%
    /tikz/ortho/du distance={#1},%
    /tikz/ortho/lr distance={#1},%
    /tikz/ortho/rl distance={#1}},%
  ortho/ud distance/.initial=+.5cm,%
  ortho/du distance/.initial=+.5cm,%
  ortho/lr distance/.initial=+.5cm,%
  ortho/rl distance/.initial=+.5cm,%
  ortho/ratio=.5,% default value
  ortho/spacing=4,% default value
}%

%BEGIN_FOLD Timer
\def\tikzext@timer@hvhline{%
  \pgf@process{\tikz@timer@start}\pgf@ya\pgf@y
  \pgf@process{\tikz@timer@end}\pgf@yc\pgf@y
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\tikzext@tikz@hvvh@timing@first pt% first quarter
    \iftikzext@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
  \else
    \ifdim\tikz@time pt>\tikzext@tikz@hvvh@timing@last pt% last quarter
      \iftikzext@tikz@hvvh@middle
        \advance\pgf@xb-1pt%
      \else
        \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
      \fi
      \advance\pgf@xb\dimexpr-\tikzext@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@yc}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb\tikzext@tikz@hvvh@timing@factor\pgf@xb%
      \advance\pgf@xb-\tikzext@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@middle}}%
    \fi\fi\tikz@marshal}
\def\tikzext@timer@vhvline{%
  \pgf@process{\tikz@timer@start}\pgf@xa\pgf@x
  \pgf@process{\tikz@timer@end}\pgf@xc\pgf@x
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\tikzext@tikz@hvvh@timing@first pt% first quarter
    \iftikzext@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
  \else
    \ifdim\tikz@time pt>\tikzext@tikz@hvvh@timing@last pt% last quarter
    \iftikzext@tikz@hvvh@middle
      \advance\pgf@xb-1pt%
    \else
      \pgf@xb\tikzext@tikz@hvvh@timing@parts\pgf@xb
    \fi
      \advance\pgf@xb by\dimexpr-\tikzext@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb=\tikzext@tikz@hvvh@timing@factor\pgf@xb
      \advance\pgf@xb by-\tikzext@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@middle}}%
      \fi\fi\tikz@marshal}%

%% collect options and nodes, coordinates and pics onpath
\let\tikz@hvvh@currentoption\pgfutil@empty
\def\tikzext@tikz@collect@hvvh@options#1[#2]{\edef\tikz@hvvh@currentoption{#2}#1}
\def\tikzext@tikz@hvh@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@hvh@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@hvh@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@hvh@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@hvh@lineto}}}}%
\def\tikzext@tikz@vhv@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@vhv@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@vhv@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@vhv@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@vhv@lineto}}}}%
\def\tikzext@tikz@ud@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@ud@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@ud@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@ud@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@ud@lineto}}}}%
\def\tikzext@tikz@du@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@du@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@du@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@du@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@du@lineto}}}}%
\def\tikzext@tikz@lr@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@lr@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@lr@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@lr@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@lr@lineto}}}}%
\def\tikzext@tikz@rl@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikzext@tikz@rl@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikzext@tikz@rl@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikzext@tikz@rl@lineto@next}{\tikz@scan@one@point\tikzext@tikz@@rl@lineto}}}}%

\def\tikzext@do@hvvh#1#2#3#4#5{%
% #1 = first kink
% #2 = second kink
% #3 = end
% #4 = timer
% #5 = tikz@shapeborder@name
  \pgfpathlineto{#1}%
  \pgfpathlineto{#2}%
  \pgfpathlineto{#3}%
  \def\tikz@timer@middle{#2}%
  \def\tikz@timer@end{#3}%
  \let\tikz@timer#4
  \edef\pgf@temp{#5}%
  \ifx\pgf@temp\pgfutil@empty
    \let\tikz@moveto@waiting\relax
  \else
    \let\tikz@moveto@waiting\pgf@temp
  \fi
  \tikz@scan@next@command}%

%% -|- operator
\def\tikzext@tikz@@hvh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb=\tikz@lastx
  \pgf@xc=\tikz@lastx
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xb}{\tikz@lasty}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \pgfutil@ifxempty\tikzext@tikz@hvvh@ratio{%
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \iftikzext@tikz@hvvh@fromcenter
            \pgf@xc\tikz@lastx
          \else
            \pgf@xc\pgf@x
          \fi
        \fi
        \ifdim\pgf@xb>\tikz@lastx
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      }{%
        \iftikzext@tikz@hvvh@fromcenter
          \tikzext@tikz@hvvh@distance\tikz@lastx
        \else
          \tikzext@tikz@hvvh@distance\pgf@x
        \fi
        \advance\tikzext@tikz@hvvh@distance-\pgf@xc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      }%
      \advance\pgf@xc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \pgfutil@ifxempty\tikzext@tikz@hvvh@ratio{%
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \pgf@xc\tikz@lastx
        \fi
        \ifdim\pgf@xb>\tikz@lastx
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      }{%
        \tikzext@tikz@hvvh@distance\tikz@lastx
        \advance\tikzext@tikz@hvvh@distance-\pgf@xc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      }%
      \advance\pgf@xc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikzext@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikzext@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% |-| operator
\def\tikzext@tikz@@vhv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx
  \pgf@yb=\tikz@lasty
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yb}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\tikzext@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \iftikzext@tikz@hvvh@fromcenter
            \pgf@yc\tikz@lasty
          \else
            \pgf@yc\pgf@y
          \fi
        \fi
        \ifdim\pgf@yb>\tikz@lasty
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      \else
        \iftikzext@tikz@hvvh@fromcenter
          \tikzext@tikz@hvvh@distance\tikz@lasty
        \else
          \tikzext@tikz@hvvh@distance\pgf@y
        \fi
        \advance\tikzext@tikz@hvvh@distance-\pgf@yc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\tikzext@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\tikzext@tikz@hvvh@distance<0pt\relax
          \pgf@yc\tikz@lasty
        \fi
        \ifdim\pgf@yb>\tikz@lasty
          \tikzext@tikz@hvvh@distance-\tikzext@tikz@hvvh@distance
        \fi
      \else
        \tikzext@tikz@hvvh@distance\tikz@lasty
        \advance\tikzext@tikz@hvvh@distance-\pgf@yc
        \tikzext@tikz@hvvh@distance\tikzext@tikz@hvvh@ratio\tikzext@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\tikzext@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikzext@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikzext@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-ud operator
\def\tikzext@tikz@@ud@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/ud distance}}%
    \iftikz@shapeborder
      \advance\pgf@y1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc<\pgf@y
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb<\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb\tikzext@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikzext@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikzext@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-du operator
\def\tikzext@tikz@@du@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/du distance}}%
    \iftikz@shapeborder
      \advance\pgf@y-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc>\pgf@y
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc-\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb>\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb-\tikzext@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikzext@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikzext@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-lr operator
\def\tikzext@tikz@@lr@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/ortho}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/lr distance}}%
    \iftikz@shapeborder
      \advance\pgf@x-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc>\pgf@x
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc-\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb>\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb-\tikzext@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikzext@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikzext@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% r-rl operator
\def\tikzext@tikz@@rl@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/ortho/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\tikzext@tikz@udlr@distance{\pgfkeysvalueof{/tikz/ortho/rl distance}}%
    \iftikz@shapeborder%
      \advance\pgf@x1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \iftikzext@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc<\pgf@x
        \iftikzext@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc\tikzext@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty%
      \ifx\pgf@temp\relax\else
        \iftikzext@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb<\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb\tikzext@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikzext@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikzext@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}%

%% a few nice to haves, use with to or edge operator
\tikzset{
  node as new start/.is if=tikzext@ortho@preflush,
  node as new start,
  ortho/install shortcuts/.style={
    *|/.style={/tikz/only vertical   second={##1}}, *|/.default=,
    |*/.style={/tikz/only vertical   first={##1}},  |*/.default=,
    *-/.style={/tikz/only horizontal second={##1}}, *-/.default=,
    -*/.style={/tikz/only horizontal first={##1}},  -*/.default=,
    |-/.style={/tikz/to path={|-(\tikztotarget)\tikztonodes}},
    -|/.style={/tikz/to path={-|(\tikztotarget)\tikztonodes}},
    -|-/.style={/tikz/horizontal vertical horizontal={##1}}, -|-/.default=,
    |-|/.style={/tikz/vertical   horizontal vertical={##1}}, |-|/.default=,
    r-du/.style={/tikz/down horizontal up={##1}}, r-du/.default=,
    r-ud/.style={/tikz/up horizontal down={##1}}, r-ud/.default=,
    r-rl/.style={/tikz/right vertical left={##1}}, r-rl/.default=,
    r-lr/.style={/tikz/left vertical right={##1}}, r-lr/.default=%
  },
  horizontal vertical/.style={to path={-|(\tikztotarget)\tikztonodes}},
  vertical horizontal/.style={to path={|-(\tikztotarget)\tikztonodes}},
  horizontal vertical horizontal/.default=,
  horizontal vertical horizontal/.style={to path={-|-[{#1}](\tikztotarget)\tikztonodes}},
  vertical horizontal vertical/.default=,
  vertical horizontal vertical/.style={to path={|-|[{#1}](\tikztotarget)\tikztonodes}},
  right vertical left/.default=,
  right vertical left/.style={to path={r-rl[{#1}](\tikztotarget)\tikztonodes]}},
  left vertical right/.default=,
  left vertical right/.style={to path={r-lr[{#1}](\tikztotarget)\tikztonodes]}},
  up horizontal down/.default=,
  up horizontal down/.style={to path={r-ud[{#1}](\tikztotarget)\tikztonodes]}},
  down horizontal up/.default=,
  down horizontal up/.style={to path={r-du[{#1}](\tikztotarget)\tikztonodes]}},
  only vertical second/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztostart{\tikztostart.north}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.south}\fi
        \else
          \edef\tikztostart{\tikztostart.south}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.north}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \let\tikzext@origtotarget\tikztotarget
        \edef\tikztotarget{[xshift={#1}]\tikztotarget\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    \pgfkeys@expanded{%
      (perpendicular cs: horizontal line through={(\tikztostart)},
                         vertical line through={(\tikztotarget)}) -- (\tikztotarget)}\tikztonodes
      \pgfextra
        \ifx\tikzext@origtotarget\pgfutil@empty\else
          \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only vertical second/.default=,
  only horizontal second/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztostart{\tikztostart.east}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.west}\fi
        \else
          \edef\tikztostart{\tikztostart.west}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.east}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \let\tikzext@origtotarget\tikztotarget
        \edef\tikztotarget{[yshift={#1}]\tikztotarget\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    \pgfkeys@expanded{%
      (perpendicular cs: vertical line through={(\tikztostart)},
                         horizontal line through={(\tikztotarget)}) -- (\tikztotarget)}\tikztonodes
    \pgfextra
      \ifx\tikzext@origtotarget\pgfutil@empty\else
        \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only horizontal second/.default=,
  only vertical first/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \pgf@ya=\pgf@y
      \iftikz@shapeborder
        \let\tikzext@origtotarget\tikztotarget
        \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
        \ifdim\pgf@ya>\tikz@lasty\relax
          \edef\tikztotarget{\tikztotarget.south}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.north}\fi
        \else
          \edef\tikztotarget{\tikztotarget.north}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.south}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \edef\tikztostart{[xshift={#1}]\tikztostart\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    expandafter(\tikztostart)
    -- (perpendicular cs: vertical line through/.expanded={(\tikztostart)},
                        horizontal line through={(\tikztotarget)})
    \tikztonodes
    \pgfextra
      \ifx\tikzext@origtotarget\pgfutil@empty\else
        \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only vertical first/.default=,
  only horizontal first/.style={to path={
    \pgfextra
      \let\tikzext@ortho@anchor\pgfutil@empty
      \let\tikzext@origtotarget\pgfutil@empty
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \pgf@xa=\pgf@x
      \iftikz@shapeborder
        \let\tikzext@origtotarget\tikztotarget
        \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)\relax
        \ifdim\pgf@xa>\tikz@lastx\relax
          \edef\tikztotarget{\tikztotarget.west}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.east}\fi
        \else
          \edef\tikztotarget{\tikztotarget.east}%
          \iftikz@shapeborder\def\tikzext@ortho@anchor{.west}\fi
        \fi
      \fi
      \def\tikz@tempa{#1}%
      \ifx\tikz@tempa\pgfutil@empty\else
        \edef\tikztostart{[yshift={#1}]\tikztostart\tikzext@ortho@anchor}%
      \fi
    \endpgfextra
    \expandafter(\tikztostart)
      -- (perpendicular cs: horizontal line through/.expanded={(\tikztostart)},
                              vertical line through={(\tikztotarget)})
    \tikztonodes \pgfextra
      \ifx\tikzext@origtotarget\pgfutil@empty\else
        \iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi\endpgfextra}},
  only horizontal first/.default=,
  only vertical first to center/.style={to path={
    \pgfextra
      \let\tikzext@origtotarget\tikztotarget
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: vertical line through={(\tikztostart)},
                                         horizontal line through={(\tikztotarget)})
    \tikztonodes \ifx\tikzext@origtotarget\pgfutil@empty\else\iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi}},
  only horizontal first to center/.style={to path={
    \pgfextra
      \let\tikzext@origtotarget\tikztotarget
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: horizontal line through={(\tikztostart)},
                                         vertical line through={(\tikztotarget)})
    \tikztonodes \ifx\tikzext@origtotarget\pgfutil@empty\else\iftikzext@ortho@preflush(\tikzext@origtotarget)\fi\fi}}%
}
\endinput
